Predicting Scores of Medical Imaging Segmentation Methods with Meta-Learning

Deep learning has led to state-of-the-art results for many medical imaging tasks, such as segmentation of different anatomical structures. With the increased numbers of deep learning publications and openly available code, the approach to choosing a model for a new task becomes more complicated, while time and (computational) resources are limited. A possible solution to choosing a model efficiently is meta-learning, a learning method in which prior performance of a model is used to predict the performance for new tasks. We investigate meta-learning for segmentation across ten datasets of different organs and modalities. We propose four ways to represent each dataset by meta-features: one based on statistical features of the images and three are based on deep learning features. We use support vector regression and deep neural networks to learn the relationship between the meta-features and prior model performance. On three external test datasets these methods give Dice scores within 0.10 of the true performance. These results demonstrate the potential of meta-learning in medical imaging.

==> draft.tex <==
%The output of the feature extractors is processed to have a single dimensions ($M^{20}_{(x,7,7) }\xrightarrow{}M^{20}_{x }$), making them similar to the statistical meta-features. First the outputs of all images in the meta subset will be averaged. Next, a set is created including one averaged metafeature per dataset. All meta-features in this set are compared to each other. If one of the feature maps at index \textit{j} has a correlation larger than $80\%$  with a feature map of another dataset at index \textit{j}, the feature maps are considered similar. This correlation threshold is empirically determined. If this is the case both meta-features will get the value: '$1$' for that feature map (\autoref{fig:filters}). If not the value for that feature map will be: '$0$'.  This will be repeated for the number of meta-features that are needed to be extracted. This process yields meta-features of sizes $512$, $2048$ and $1024$ for VGG16, ResNet50 and MobileNetV1 features extractors respectively. 
\section{text from methods}

Four different types of metafeatures are defined. The first type is the statistical metafeature. Choice and validation of this metafeature is fully manual. Therefore it is interesting to compare these metafeatures with metafeatures generated using a automated approach. The remainin three types of metafeatures are generated with a deep learning based apporach, each with a different type of base architecture.   

The requirement of this finetuning is that the encoder/feature extractor should yield a specific set of features for a dataset. The features do not have to hold a specific meaning. For example, the features do not need to lead to classification or segmentation of images. This nuance allows circumventing the use of labelled data. Using labelled data in the metafeature extraction is not preferred, as one of the goals of the meta-learning method is to do predictions on datasets with no known labels based on the metafeatures of these datasets. To apply the proposed method a type of target data is needed perform finetuning.

This target data is created by using the $10^{th}$ percentile of the data as a target mask. The $10^{th}$ percentile of an image captures the general structural features of an image in both CT and MR images. Predicting the $10^{th}$ percentile of an image does not yield a useful result in terms of segmentation. However this is not the objective, because that is to extract the unique features of the image which is hypothesised to be possible using this method.

 
 Three models pretrained on ImageNet were used. A selection criteria for the models is that they are available on the Keras library \cite{chollet2015keras}, thus guaranteeing a quality baseline for the model weights. Furthermore the methods need to be have different architectures to be able to do a comparison between methods. 

\section{Text from intro}
Both these examples show a move to a more efficient use of available information, but are centered around the creation of new models.  The no free lunch theorem tells us there will not be one model which performs the best on all problems \cite{NFL2002}. Knowing beforehand how a given model will perform on the new task you try to solve can reduce the number of potential models you have to train and evaluate before finding the optimal model for that task. Meta-learning is a technique that makes it possible to make such predictions on models. 

Meta-learning is type of learning that guides its learning process through the use of prior information. The concept of meta-learning originates from psychology, where meta-learning is viewed as learning based on the requirements of a specific task . This is a concept that everyone uses in their everyday life. 


The lack of research into applying meta-learning in medical imaging can be attributed to multiple reasons. First, it could be explained by the relatively high resolution and dimensionality (2D, 3D, 4D) of medical images, the sometimes small regions of interest, changing field of view and uncertainty in assessment (even of experts). On the other side, problems in medical image analysis share the same characteristics; There is a limited amount of imaging modalities and anatomy is (most often) within certain bounds, as well as the scale differences between humans.

Another limiting factor in the usage of meta-learning is data availability. As mentioned, deep learning in medical imaging only exists for a couple years. To apply meta-learning, prior dataset performance on models should be available. Over the last years there is an increase in public medical-imaging datasets and the increasing usage of GitHub amongst deep learning practitioners in medical imaging increases the accessibility to prior model information \cite{greenspan2016guest}.
Meta-learning can potentially be used in this field to safeguard against inefficient development processes.  Currently data preparation, model choices and hyper parameter tuning take a considerable amount of manual labour, because the current workflow for solving a medical image analysis problem is more or less following a trial and error method. Several methods are tried, which might not be computationally efficient. In many cases this is not a direct problem, because 1) the tasks might not be time-sensitive or 2) memory usage might not be an issue. However with the increasing amount of new deep learning solutions and the ease of finding them online and applying them, the trial-and-error way of doing research can get increasingly inefficient. Optimising this can  lead to faster advances in the medical image analysis field.  In summary, when looking at the data and problems that are being solved in medical imaging using deep learning there is a case for using meta-learning.


\subsection{Project goals}

In this project we propose a meta-learning method on medical image segmentation. This is a suitable sub domain to choose, because the majority of research papers published over the last years on deep learning for medical image analysis are on medical image segmentation \cite{LITJENS201760}. Furthermore medical image segmentation is not modality or location dependent. This makes assembling assembling a meta-learning dataset easier and less bound to constraints. Moreover, most of the state-of-the-art models in medical image segmentation are deep learning based solutions. However there is not one method that yields the best in all (or most) problems. 
A method that could quantify the estimated performance of a model on a specific dataset could be of great value. This would mean that the step where you choose a deep learning  model to solve your problem is (partly) automated.

The goal of this project is to show how past performance of deep learning algorithms, combined with meta-information of a new dataset can yield a good estimation of the performance, and thus viability, of said algorithm on a new dataset. This can enable more efficient use of time and resources. 
That should be achieved by first showing that problems in medical image analysis all have specific characteristics, but also share some information. Secondly a meta-learning prediction method should be created. Lastly the prospects and possibilities of meta-learning in medical image analysis should be analysed to be able to identify bottlenecks, challenges and opportunities for meta-learning in medical imaging.

\tom{template content}
\section{First Section}
\subsection{A Subsection Sample}
Please note that the first paragraph of a section or subsection is
not indented. The first paragraph that follows a table, figure,
equation etc. does not need an indent, either.

Subsequent paragraphs, however, are indented.

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|} 
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
\includegraphics[width=\textwidth]{fig1.eps}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}
For citations of references, we prefer the use of square brackets
and consecutive numbers. Citations using labels or the author/year
convention are also acceptable. The following bibliography provides
a sample reference list with entries for journal
articles~\cite{ref_article1}, an LNCS chapter~\cite{ref_lncs1}, a
book~\cite{ref_book1}, proceedings without editors~\cite{ref_proc1},
and a homepage~\cite{ref_url1}. Multiple citations are grouped
\cite{ref_article1,ref_lncs1,ref_book1},
\cite{ref_article1,ref_book1,ref_proc1,ref_url1}.
%
% ---- Bibliography ----
%
% BibTeX users should specify bibliography style 'splncs04'.
% References will then be sorted and formatted in the correct style.
%
% \bibliographystyle{splncs04}
% \bibliography{mybibliography}
%
\begin{thebibliography}{8}
\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor,
F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
Location (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, Location (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
Oct 2017
\end{thebibliography}

==> supplementaryMaterial.tex <==
\section{Supplementary material}

\subsection{Statistical metafeatures}
List of 33 statistical features used to compose the statistical metafeatures.
\setcounter{table}{0}
\renewcommand{\thetable}{S1.\arabic{table}}
\label{appendix:stat}
\begin{table}[!h]
\centering
\resizebox{\textwidth/3}{!}{
\begin{tabular}{l}
\hlineB{4}
\textbf{Statistical metafeatures}\\\hlineB{4}
Number of instances\\\hline
Voxel value M\\\hline
Voxel value STD\\\hline
Voxel value CVAR\\\hline
Skew M\\\hline
STD\\\hline
Skew CVAR\\\hline
Kurtosis M\\\hline
Kurtosis STD\\\hline
Kurtosis CVAR\\\hline
Entropy M\\\hline
Entropy STD\\\hline
Entropy CVAR\\\hline
Median M\\\hline
Median STD\\\hline
Mutual information M\\\hline
Mutual information STD\\\hline
Mutual information CVAR\\\hline
Mutual information maximum value\\\hline
Correlation M\\\hline
Correlation STD\\\hline
Correlation CVAR\\\hline
Sparsity M\\\hline
Sparsity STD\\\hline
Sparsity CVAR\\\hline
Slice size M\\\hline
Slice size STD\\\hline
Slice size CVAR\\\hline
Number of slices M\\\hline
Number of slices STD \\\hline
Number of slices CVAR\\\hline
Equivalent number of features\\\hline
Noise signal ratio\\\hline
\end{tabular}}\\

\captionsetup{width=0.8\textwidth/2}
\caption{Statistical metafeatures used in the Support Vector Regression method. M = mean, STD = standard deviation, CVAR = coefficient of variation. }



\end{table}

\clearpage

\subsection{Full results SVR meta-learner}
Full results of SVR meta-learner. Consists of: MAE scores per MSD dataset, MAE scores per MSD challenge participant, method rank correlation and task rank correlation. 
\label{appendix:svrtot}
\setcounter{table}{0}
\renewcommand{\thetable}{S2.\arabic{table}}
\begin{table}[htp]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|ll|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{MSD datasets $\downarrow$}} & \multicolumn{8}{c|}{Mean absolute error $\downarrow$} \\ \cline{3-10} 
\multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{Classical} & \multicolumn{2}{c|}{VGG16} & \multicolumn{2}{c|}{ResNet50} & \multicolumn{2}{c|}{MobileNetV1} \\ \cline{3-10} 
\multicolumn{2}{|l|}{Meta-learner $\rightarrow$} & \multicolumn{1}{c|}{SVR} & DNN & \multicolumn{1}{c|}{SVR} & DNN & \multicolumn{1}{c|}{SVR} & DNN & \multicolumn{1}{c|}{SVR} & DNN \\ \hline
1  & Braintumor     & $0.17\pm0.05$ & $0.06\pm0.06$ & $0.07\pm0.01$ & $0.09\pm0.01$ & $0.08\pm0.01$ & $0.22\pm0.06$ & $0.14\pm0.01$ & $0.22\pm0.06$ \\ \hline
2  & Heart          & $0.07\pm0.01$ & $0.18\pm0.05$ & $0.06\pm0.05$ & $0.09\pm0.01$ & $0.14\pm0.06$ & $0.05\pm0.01$ & $0.15\pm0.07$ & $0.11\pm0.02$ \\ \hline
3  & Liver          & $0.29\pm0.15$ & $0.55\pm0.25$ & $0.08\pm0.17$ & $0.03\pm0.00$ & $0.11\pm0.10$ & $0.04\pm0.00$ & $0.28\pm0.15$ & $0.24\pm0.06$ \\ \hline
4  & Hippocampus    & $0.07\pm0.01$ & $0.09\pm0.01$ & $0.04\pm0.07$ & $0.07\pm0.01$ & $0.08\pm0.07$ & $0.10\pm0.01$ & $0.06\pm0.07$ & $0.07\pm0.01$ \\ \hline
5  & Prostate       & $0.14\pm0.03$ & $0.27\pm0.09$ & $0.09\pm0.00$ & $0.21\pm0.05$ & $0.05\pm0.00$ & $0.07\pm0.01$ & $0.04\pm0.00$ & $0.05\pm0.01$ \\ \hline
6  & Lung           & $0.09\pm0.01$ & $0.09\pm0.01$ & $0.21\pm0.11$ & $0.23\pm0.06$ & $0.17\pm0.07$ & $0.10\pm0.02$ & $0.09\pm0.09$ & $0.09\pm0.02$ \\ \hline
7  & Pancreas       & $0.19\pm0.03$ & $0.07\pm0.01$ & $0.10\pm0.01$ & $0.09\pm0.01$ & $0.06\pm0.01$ & $0.09\pm0.01$ & $0.05\pm0.01$ & $0.16\pm0.04$ \\ \hline
8  & Hepatic vessel & $0.12\pm0.01$ & $0.10\pm0.05$ & $0.26\pm0.03$ & $0.21\pm0.06$ & $0.13\pm0.04$ & $0.21\pm0.05$ & $0.13\pm0.06$ & $0.09\pm0.02$ \\ \hline
9  & Spleen         & $0.46\pm0.18$ & $0.40\pm0.18$ & $0.08\pm0.14$ & $0.03\pm0.00$ & $0.10\pm0.11$ & $0.03\pm0.00$ & $0.21\pm0.10$ & $0.12\pm0.02$ \\ \hline
10 & Colon          & $0.54\pm0.23$ & $0.56\pm0.32$ & $0.31\pm0.28$ & $0.34\pm0.13$ & $0.31\pm0.25$ & $0.33\pm0.15$ & $0.36\pm0.30$ & $0.25\pm0.08$ \\ \hline
\textbf{} & \textbf{Total} & \multicolumn{1}{l|}{\textbf{$0.21\pm0.08$}} & \textbf{$0.24\pm0.09$} & \multicolumn{1}{l|}{\textbf{$0.13\pm0.09$}} & \textbf{$0.14\pm0.04$} & \multicolumn{1}{l|}{\textbf{$0.12\pm0.07$}} & \textbf{$0.12\pm0.03$} & \multicolumn{1}{l|}{\textbf{$0.15\pm0.09$}} & \textbf{$0.14\pm0.03$} \\ \hline
\end{tabular}%
}
\caption{Total MAE results of cross-validation on MSD datasets per dataset using a SVR meta-learner}
\label{tab:maetotmsvr}
\end{table}
\begin{table}[htp]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{Participants $\downarrow$} & \multicolumn{8}{c|}{Mean absolute error $\downarrow$} \\ \cline{2-9} 
 & \multicolumn{2}{c|}{Clasical} & \multicolumn{2}{c|}{VGG16} & \multicolumn{2}{c|}{ResNet50} & \multicolumn{2}{c|}{MobileNetV1} \\ \cline{2-9} 
Meta-learner $\rightarrow$ & SVR & DNN & SVR & DNN & SVR & DNN & SVR & DNN \\ \hline
Participant 1  & $0.25\pm0.08$ & $0.29\pm0.29$ & $0.08\pm0.11$ & $0.11\pm0.02$ & $0.18\pm0.10$ & $0.20\pm0.08$ & $0.19\pm0.12$ & $0.21\pm0.06$ \\ \hline
Participant 2  & $0.18\pm0.06$ & $0.19\pm0.19$ & $0.11\pm0.05$ & $0.11\pm0.02$ & $0.10\pm0.05$ & $0.12\pm0.03$ & $0.13\pm0.05$ & $0.13\pm0.02$ \\ \hline
Participant 3  & $0.20\pm0.05$ & $0.21\pm0.07$ & $0.12\pm0.06$ & $0.10\pm0.02$ & $0.11\pm0.05$ & $0.11\pm0.02$ & $0.13\pm0.06$ & $0.13\pm0.03$ \\ \hline
Participant 4  & $0.27\pm0.09$ & $0.24\pm0.10$ & $0.11\pm0.14$ & $0.14\pm0.03$ & $0.14\pm0.12$ & $0.17\pm0.04$ & $0.18\pm0.14$ & $0.13\pm0.03$ \\ \hline
Participant 5  & $0.19\pm0.70$ & $0.21\pm0.05$ & $0.12\pm0.06$ & $0.12\pm0.03$ & $0.11\pm0.05$ & $0.09\pm0.02$ & $0.12\pm0.06$ & $0.11\pm0.02$ \\ \hline
Participant 6  & $0.24\pm0.10$ & $0.25\pm0.11$ & $0.13\pm0.09$ & $0.15\pm0.03$ & $0.14\pm0.08$ & $0.11\pm0.02$ & $0.19\pm0.10$ & $0.18\pm0.04$ \\ \hline
Participant 7  & $0.21\pm0.07$ & $0.29\pm0.09$ & $0.16\pm0.12$ & $0.20\pm0.05$ & $0.15\pm0.09$ & $0.12\pm0.03$ & $0.15\pm0.11$ & $0.13\pm0.02$ \\ \hline
Participant 8  & $0.15\pm0.03$ & $0.16\pm0.02$ & $0.07\pm0.03$ & $0.07\pm0.01$ & $0.09\pm0.03$ & $0.07\pm0.01$ & $0.12\pm0.03$ & $0.11\pm0.02$ \\ \hline
Participant 9  & $0.24\pm0.10$ & $0.23\pm0.08$ & $0.14\pm0.08$ & $0.15\pm0.03$ & $0.12\pm0.07$ & $0.08\pm0.01$ & $0.22\pm0.08$ & $0.15\pm0.04$ \\ \hline
Participant 10 & $0.21\pm0.08$ & $0.27\pm0.10$ & $0.17\pm0.10$ & $0.19\pm0.06$ & $0.14\pm0.08$ & $0.16\pm0.06$ & $0.13\pm0.10$ & $0.12\pm0.02$ \\ \hline
Participant 11 & $0.24\pm0.09$ & $0.26\pm0.14$ & $0.17\pm0.09$ & $0.18\pm0.07$ & $0.14\pm0.08$ & $0.16\pm0.06$ & $0.15\pm0.1$  & $0.18\pm0.05$ \\ \hline
Participant 12 & $0.26\pm0.10$ & $0.26\pm0.15$ & $0.17\pm0.11$ & $0.20\pm0.06$ & $0.16\pm0.09$ & $0.16\pm0.04$ & $0.17\pm0.11$ & $0.15\pm0.04$ \\ \hline
Participant 13 & $0.18\pm0.06$ & $0.23\pm0.60$ & $0.11\pm0.06$ & $0.11\pm0.02$ & $0.01\pm0.05$ & $0.12\pm0.03$ & $0.14\pm0.06$ & $0.15\pm0.03$ \\ \hline
Participant 14 & $0.15\pm0.04$ & $0.18\pm0.03$ & $0.08\pm0.04$ & $0.09\pm0.01$ & $0.09\pm0.03$ & $0.08\pm0.01$ & $0.10\pm0.04$ & $0.10\pm0.02$ \\ \hline
Participant 15 & $0.17\pm0.04$ & $0.19\pm0.04$ & $0.09\pm0.05$ & $0.08\pm0.01$ & $0.10\pm0.04$ & $0.10\pm0.01$ & $0.12\pm0.05$ & $0.10\pm0.02$ \\ \hline
Participant 16 & $0.22\pm0.09$ & $0.26\pm0.12$ & $0.15\pm0.08$ & $0.14\pm0.04$ & $0.12\pm0.07$ & $0.12\pm0.03$ & $0.14\pm0.09$ & $0.13\pm0.03$ \\ \hline
Participant 17 & $0.20\pm0.08$ & $0.24\pm0.09$ & $0.13\pm0.08$ & $0.13\pm0.04$ & $0.12\pm0.07$ & $0.11\pm0.03$ & $0.14\pm0.08$ & $0.16\pm0.04$ \\ \hline
Participant 18 & $0.28\pm0.12$ & $0.31\pm0.15$ & $0.21\pm0.15$ & $0.25\pm0.07$ & $0.15\pm0.11$ & $0.22\pm0.07$ & $0.19\pm0.13$ & $0.22\pm0.06$ \\ \hline
Participant 19 & $0.22\pm0.08$ & $0.25\pm0.09$ & $0.16\pm0.09$ & $0.15\pm0.05$ & $0.12\pm0.08$ & $0.11\pm0.02$ & $0.14\pm0.09$ & $0.13\pm0.03$ \\ \hline
\textbf{Total} & \textbf{$0.21\pm0.08$} & \textbf{$0.24\pm0.10$} & \textbf{$0.13\pm0.09$} & \textbf{$0.14\pm0.04$} & \textbf{$0.13\pm0.07$} & \textbf{$0.13\pm0.03$} & \textbf{$0.15\pm0.09$} & \textbf{$0.14\pm0.03$} \\ \hline
\end{tabular}%
}
\caption{Total MAE results of cross-validation on MSD datasets per participant using a SVR meta-learner}
\label{tab:maetotsvr}
\end{table}
\clearpage

==> table_testtrue.tex <==
\begin{table}[!h]
\resizebox{\textwidth/2-5pt}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l}
\multicolumn{2}{l|}{} & \multicolumn{2}{l|}{Liver (LiTS)} & \multicolumn{2}{l|}{Heart (ACDC)} & \multicolumn{2}{l}{Liver (CHAOS)} \\ \cline{3-8}
\multicolumn{2}{l|}{True model result $\xrightarrow{}$} & \multicolumn{2}{c|}{0.96} & \multicolumn{2}{c|}{0.96} & \multicolumn{2}{c}{0.89} \\ \hline
\multicolumn{2}{l|}{Feature selection $\downarrow$} & SVR & DNN & SVR & DNN & SVR & DNN \\ \hline
\multirow{2}{*}{Statistical} & Yes & 0.87 & 0.99 & 0.80 & 0.96 & 0.95 & 0.95 \\ \cline{2-8} 
 & No & 0.87 & 0.82 & 0.80 & 0.8 & 0.90 & 0.85 \\ \hline
\multirow{2}{*}{VGG16} & Yes & 0.76 & 0.83 & 0.74 & 0.91 & 0.74 & 0.9 \\ \cline{2-8} 
 & No & 0.76 & 1.00 & 0.76 & 1.00 & 0.76 & 1.00 \\ \hline
\multirow{2}{*}{ResNet50} & Yes & 0.73 & 0.46 & 0.73 & 0.94 & 0.74 & 0.95 \\ \cline{2-8} 
 & No & 0.75 & 1.00 & 0.75 & 0.94 & 0.75 & 1.00 \\ \hline
\multirow{2}{*}{MobileNetV1} & Yes & 0.82 & 0.97 & 0.75 & 0.83 & 0.82 & 0.96 \\ \cline{2-8} 
 & No & 0.76 & 1.00 & 0.76 & 0.01 & 0.76 & 1.00
\end{tabular}%
}
\caption{Prediction result of SVR and DNN meta-learners on test datasets for different types of metafeatures.}
\label{tab:testtrueresult}
\end{table}


==> todo.tex <==
TODO list
Tom
- resultaten insert
- methode beknopter 
    - deep learning feature averaging uitleggen
- experimental setup
 - dataset description
 - figuren verbeteren
- tabel met alleen resultaat van model uit test set
- discussiepunten
- methods notatie aanpassen
- bij experimental setup of result:
    alleen task specific features resultaat? 

- hoe is de related work anders dan wat wij doen? (1.1)

Veronika

- introductie korter
- figuur meta-learning system




Done



